$R(J/\psi)$ and $B_c^- \rightarrow J/\psi \ell^-\bar{\nu}_\ell$ Lepton Flavor Universality Violating Observables from Lattice QCD

We use our lattice QCD computation of the $B_c\rightarrow J/\psi$ form factors to determine the differential decay rate for the semitauonic decay channel and construct the ratio of branching fractions $R(J/\psi) = \mathcal{B}(B_c^- \rightarrow J/\psi \tau^-\bar{\nu}_\tau)/\mathcal{B}(B_c^- \rightarrow J/\psi \mu^-\bar{\nu}_\mu)$. We find $R(J/\psi) = 0.2582(38)$ and give an error budget. We also extend the relevant angular observables, which were recently suggested for the study of lepton flavor universality violating effects in $B\rightarrow D^*\ell\nu$, to $B_c \rightarrow J/\psi\ell\nu$ and make predictions for their values under different new physics scenarios.

==> acktext <==

\subsection*{\bf{Acknowledgements}}

We are grateful to the MILC collaboration for the use of
their configurations and code. 
We thank C. Bouchard, B. Colquhoun, J. Koponen, P. Lepage, 
E. McLean and C. McNeile for useful discussions.
Computing was done on the Cambridge service for Data 
Driven Discovery (CSD3), part of which is operated by the 
University of Cambridge Research Computing on behalf of 
the DIRAC 
HPC Facility of the Science and Technology Facilities 
Council (STFC). The DIRAC component of CSD3 was funded by 
BEIS capital funding via STFC capital grants ST/P002307/1 and 
ST/R002452/1 and STFC operations grant ST/R00689X/1. 
DiRAC is part of the national e-infrastructure.  
We are grateful to the CSD3 support staff for assistance.
Funding for this work came from the UK
Science and Technology Facilities Council grants 
ST/L000466/1 and ST/P000746/1.

